Harnessing the polymer-particle duality of ultra-soft nanogels to stabilise smart emulsions

Micro- and nanogels are widely used to stabilise emulsions and simultaneously implement their responsiveness to the external stimuli. One of the factors that improves the emulsion stability is the nanogel softness. Here, we study how the softest nanogels that can be synthesised with precipitation polymerisation of N-isopropylacrylamide (NIPAM), the ultra-low crosslinked (ULC) nanogels, stabilise oil-in-water emulsions. We show that ULC nanogels can efficiently stabilise emulsions already at low mass concentrations. These emulsions are resistant to droplet flocculation, stable against coalescence, and can be easily broken upon an increase in temperature. The resistance to flocculation of the ULC-stabilised emulsion droplets is similar to the one of emulsions stabilised by linear pNIPAM. In contrast, the stability against coalescence and the temperature-responsiveness closely resemble the one of emulsions stabilised by regularly crosslinked pNIPAM nanogels. The reason for this combination of properties is that ULC nanogels can be thought of as colloids in between flexible macromolecules and particles. As a polymer, ULC nanogels can efficiently stretch at the interface and cover it uniformly. As a regularly crosslinked nanogel particle, ULC nanogels protect emulsion droplets against coalescence by providing a steric barrier and rapidly respond to changes in external stimuli thus breaking the emulsion. This polymer-particle duality of ULC nanogels can be exploited to improve the properties of emulsions for various applications, for example in heterogeneous catalysis or in food science.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
